FairNN- Conjoint Learning of Fair Representations for Fair Decisions

In this paper, we propose FairNN a neural network that performs joint feature representation and classification for fairness-aware learning. Our approach optimizes a multi-objective loss function in which (a) learns a fair representation by suppressing protected attributes (b) maintains the information content by minimizing a reconstruction loss and (c) allows for solving a classification task in a fair manner by minimizing the classification error and respecting the equalized odds-based fairness regularized. Our experiments on a variety of datasets demonstrate that such a joint approach is superior to separate treatment of unfairness in representation learning or supervised learning. Additionally, our regularizers can be adaptively weighted to balance the different components of the loss function, thus allowing for a very general framework for conjoint fair representation learning and decision making.

==> ans.tex <==
1. - Our network learns fair representation and fair classifier jointly in an end-to-end manner. (2 steps vs. 1 step)

   - comparing with Fair-PCA, we could see that having a fair representation only is not enough for a fair classification
   
   - balance the fairness and predictive performance well 

2. data transformation = one-hot encoding?

We want to select the target item from different nominal values, but not simply reconstruct the id number of each nominal value. The additional cross-entropy loss function is designed for nominal attributes.

Experiments in Fig.~\ref{fig:mul_nor_loss}.

3.The initial idea of Preferential Sampling is to create a discrimination-free training set. But we use the similar strategy for solving the class-imbalance problem. It is included in the experiment section but not the method section. See Fig.~\ref{fig:example_ps}

\begin{figure}[!htbp]
	\centering
	\includegraphics[height= 6cm, width = 12cm]{pic/P_sampling_ae.png}
	\caption[Preferential sampling]
	{We rank the instances using prediction scores, remove several instances of DN and FN, and duplicate several instances of DP and FP.}
	\label{fig:example_ps}
\end{figure}

4. error rate

5.

6. See ~\ref{subsec:ablation}

\textbf{Contributions} Our network learns a fair representation and a fair classifier jointly in an end-to-end manner. Experiments show that our method could balance the fairness and predictive performance well.
